On the Benefits of Uncertainty Estimation for Species Classification: A Case Study on Optimizing Expert re-Annotation

Automated identification of diatoms from microscopic images is a cornerstone of large-scale freshwater biomonitoring, yet the high diversity of species and strong class imbalance pose significant challenges for reliable classification. In this study, we develop a ResNet-18 baseline for a 759-class diatom dataset and investigate how calibrated confidence estimates support selective classification to reduce expert workload without sacrificing taxonomic integrity. While the initial model exhibits overconfidence with an Expected Calibration Error (ECE) of 0.117, post-hoc temperature scaling (T = 2.12) dramatically improves reliability, lowering the ECE to 0.055.By leveraging these calibrated probabilities within a triage framework, we demonstrate that a Selective Macro-F1 score of 99.01% can be maintained at 66.2% coverage (rejection threshold $\tau$ = 0.934). Qualitative analysis reveals that the system effectively functions as an intelligent filter, consistently deferring rare taxa-such as AAMB and AASI-and ambiguous morphologies for expert review. Our findings, supported by the torch-uncertainty framework, highlight the potential of simple calibration techniques to make automated diatom identification practical and robust, prioritizing the preservation of rare species metrics essential for ecological assessment. To support reproducibility, our code, environment specifications, and calibration results are available anonymously at https://anonymous.4open. science/r/greenprwksp-B53D/README.

==> sections_sam3/abstract.tex <==
\begin{abstract}

Automated diatom analysis is an important tool for water quality monitoring, but it remains difficult due to the large morphological diversity of diatom species and the limited effectiveness of specialized deep learning solutions. This paper evaluates the Segment Anything Model 3 (SAM3) for two independent tasks: species classification and text-prompted segmentation. For classification, a frozen encoder is combined with a Spatially Localized Channel Attention (SLCA) module and a convolutional classification head, reaching 95.57\% top-1 accuracy on a 102-class dataset. For segmentation, text prompts of varying specificity are evaluated, showing that short, visually grounded morphological descriptions consistently outperform species-name or detailed prompts. Two main failure modes are identified: complete non-detection and interior hollowing. 
These findings demonstrate the potential of vision foundation models for biological microscopy, while highlighting clear limitations in zero-shot semantic transfer to specialized domains.

\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}

==> sections_sam3/methodology.tex <==
\section{Methodology}

We build two independent evaluation pipelines on SAM3 to assess its capability for diatom analysis. The first pipeline addresses species classification: we use SAM3's frozen encoder to produce feature maps, which are then processed by a lightweight attention-based head to predict the species class. The second pipeline addresses segmentation: we apply SAM3 directly to the input images, conditioned on text prompts describing diatom morphology. All experiments were conducted on an NVIDIA RTX 3090 GPU. Figure~\ref{fig:pipeline} illustrates both pipelines.

%--- TikZ Pipeline Diagram ---
\begin{figure}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  node distance=0.55cm and 0.65cm,
  box/.style={draw, rounded corners=3pt, minimum width=2.1cm, minimum height=0.7cm,
              align=center, font=\small, fill=blue!10, draw=blue!50!black},
  redbox/.style={draw, rounded corners=3pt, minimum width=2.1cm, minimum height=0.7cm,
                 align=center, font=\small, fill=red!10, draw=red!60!black},
  greenbox/.style={draw, rounded corners=3pt, minimum width=2.1cm, minimum height=0.7cm,
                   align=center, font=\small, fill=green!10, draw=green!50!black},
  arr/.style={-Stealth, thick},
  lbl/.style={font=\scriptsize\itshape, text=black}
]
% Nodes
\node[box]     (img)     {Grayscale\\Input $x_i$};
\node[box, right=of img] (enc)  {Encoder\\(frozen)};
\node[box, right=of enc] (feat) {Feature Maps\\$F_i$};

\node[redbox,   right=0.5cm and 0.65cm of feat] (slca) {SLCA\\Module};

\node[box, below=2cm of img, xshift=4cm] (img2) {Grayscale\\Input $x_i$};
\node[greenbox, right=of img2] (dec)  {SAM3};

\node[redbox,   right=of slca] (head)   {Classification\\Head};
\node[greenbox, below=0.45cm  of dec]   (prompt) {Text Prompt\\$p_i$};

\node[redbox,   right=of head]   (cls)  {Species\\Label $\hat{y}_i$};
\node[greenbox, right=of dec]    (mask) {Binary\\Mask $\hat{M}_i$};

% Arrows
\draw[arr] (img)  -- (enc);
\draw[arr] (enc)  -- (feat);
\draw[arr] (feat) -- (slca);
\draw[arr] (slca)   -- (head);
\draw[arr] (head)   -- (cls);

\draw[arr] (img2)  -- (dec);
\draw[arr] (prompt) -- (dec);
\draw[arr] (dec)    -- (mask);

% Labels
\node[lbl, above=0.08cm of img]  {Task 1: Classification};
\node[lbl, above=0.08cm of img2]  {Task 2: Segmentation};
\end{tikzpicture}
}
\caption{Evaluation pipelines}
\label{fig:pipeline}
\end{figure}


\subsection{Dataset}

The dataset contains 10,660 grayscale microscopy images organized into 102 classes: 100 diatom species, one debris class, and one fragment class. Class sizes range from 40 to 305 images per species. The debris and fragment classes each contain 100 images. Images are centered on a single diatom specimen, which simplifies the learning problem but differs from real-world slides containing multiple organisms. Formally:
\[
\mathcal{D} = \{(x_i, y_i)\}_{i=1}^{N},\quad N = 10{,}660,\quad y_i \in \{1,\dots,102\}
\]
A stratified split reserves 1,602 images for testing; the remainder is used for training and validation.


\subsection{Pipeline 1: Feature Extraction and Classification}


\subsubsection{Feature Extraction}

The grayscale image $x_i$ is passed through the frozen encoder $f_\theta$, producing a dense feature tensor:
\[
F_i = f_\theta(x_i) \in \mathbb{R}^{C \times H' \times W'}
\]

The encoder is kept frozen throughout all experiments for three reasons: (i)~to leverage rich representations from large-scale pretraining~\cite{sam_feature}; (ii)~to enable offline feature precomputation, reducing training time significantly; and (iii)~to avoid overfitting given the moderate dataset size. We compare two frozen encoders(SAM2 and SAM3) and an end-to-end ResNet-18 baseline.

\subsubsection{Classification with SLCA}

Diatom species are distinguished by subtle, spatially distributed morphological features such as striae patterns and valve symmetry. Standard Global Average Pooling (GAP) discards spatial relationships entirely, losing exactly the positional information that encodes these cues. We therefore adopt the Spatially Localized Channel Attention (SLCA) mechanism from Gu~et~al.~\cite{sam_feature}, which reweights feature channels while preserving spatial locality.

SLCA first applies Spatial Local Average Pooling (SLAP) to retain local spatial context. The result passes through two $1\times1$ convolutional layers with channel reduction ratio~$r$, a ReLU activation, and a sigmoid to produce channel-wise attention weights:
\[
A_i = \sigma\!\left(\mathrm{Conv}_2\!\left(\mathrm{ReLU}\!\left(\mathrm{Conv}_1\!\left(\mathrm{SLAP}(F_i)\right)\right)\right)\right)
\]
The attention map is applied to the original feature map by element-wise multiplication:
\[
F_i^{att} = F_i \odot A_i
\]
The attended features $F_i^{att}$ are then processed by a convolutional classification head that preserves spatial inductive biases, followed by GAP and a fully connected classifier:
\[
\hat{y}_i = \mathrm{Softmax}\!\left(\mathrm{FC}\!\left(\mathrm{GAP}(F_i^{att})\right)\right)
\]

Only the SLCA module and the classification head are trained; the encoder remains frozen. Figure~\ref{fig:slca} shows the data flow.

%--- TikZ SLCA Diagram ---
\begin{figure}[htbp]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  node distance=0.4cm and 0.45cm,
  op/.style={draw, rounded corners=2pt, minimum width=1.6cm, minimum height=0.6cm,
             align=center, font=\small, fill=orange!15, draw=orange!70!black},
  arr/.style={-Stealth, thick},
  mul/.style={circle, draw, minimum size=0.32cm, font=\small, fill=yellow!30}
]
\node[op]                    (fi)   {$F_i$};
\node[op, right=of fi]       (slap) {SLAP};
\node[op, right=of slap]     (c1)   {Conv$_1$\\$1\!\times\!1$};
\node[op, right=of c1]       (relu) {ReLU};
\node[op, right=of relu]     (c2)   {Conv$_2$\\$1\!\times\!1$};
\node[op, right=of c2]       (sig)  {$\sigma$};
\node[mul, right=of sig]     (x)    {$\odot$};
\node[op, right=of x]        (att)  {$F_i^{att}$};
\node[op, below right=0.45cm and -0.3cm of att] (gap) {GAP};
\node[op, right=of gap]      (fc)   {FC};
\node[op, right=of fc]       (out)  {$\hat{y}_i$};

\draw[arr] (fi)--(slap)--(c1)--(relu)--(c2)--(sig)--(x)--(att);
\draw[arr] (fi.south) -- ++(0,-0.35) -| (x.south);
\draw[arr] (att.south) -- ++(0,-0.28) -- (gap.north);
\draw[arr] (gap)--(fc)--(out);
\end{tikzpicture}
}
\caption{SLCA data flow}
\label{fig:slca}
\end{figure}


\subsection{Pipeline 2: Prompt-Guided Segmentation}


\subsubsection{Design and Motivation}

The segmentation pipeline operates independently from classification.SAM3's mask decoder receives the raw grayscale input image and a natural-language prompt describing the target diatom.

Conceptually, we initially considered coupling both pipelines: using the classifier's species prediction to generate a specialized segmentation prompt that might improve detection. This coupling seemed appealing: many diatom species have similar shapes, and we expected the classifier to sometimes confuse related species. A species-specific prompt might help the decoder locate the correct morphological structure despite classification errors.

However, experiments revealed this coupling to be both unnecessary and ineffective. The classifier achieved 95.57\% accuracy with minimal inter-species confusion, eliminating the error-correction motivation. Consequently, the two pipelines remain fully independent in our final framework.

\subsubsection{Text Prompts and Generation}

Each image is segmented using a text prompt derived from the ground-truth species label. To test how prompt design affects segmentation, we generated five prompt types at varying specificities for each species, summarized in Table~\ref{tab:prompt_types}.

\begin{table}[htbp]
\centering
\caption{Prompt types used for segmentation evaluation.}
\label{tab:prompt_types}
\begin{tabular}{c l}
\hline
\textbf{Prompt Type} & \textbf{Description} \\
\hline
Minimal & “diatom” \\
Species Name & Exact species label \\
Simple Morphology & Short description \\
Detailed Morphology & Full structural description \\
Noisy & Incorrect or incomplete prompt \\
\hline
\end{tabular}
\end{table}



Prompt construction follows a standardized procedure. The species name is provided to GPT-4.5 along with instructions to generate a description at the desired specificity level, using a fixed template.

The segmentation itself is formalized as follows. Given an input image $x_i$ and an associated text prompt $p_i$, the SAM3 mask decoder produces a binary mask:
\[
\hat{M}_i = g_\phi(x_i,\, p_i)
\]


\subsection{Ablation Studies}


Two ablation studies are conducted. First, we compare four classification head designs: a basic fully connected classifier, a convolutional ResNet-style head, and both combined with SLCA. This isolates the contribution of spatial structure preservation and channel attention. Second, we compare segmentation performance across all five prompt types to characterize how prompt vocabulary and specificity affect SAM3's decoder.


\subsection{Evaluation Metrics}


\paragraph{Classification metrics}

\begin{enumerate}
\item \textbf{Top-1 Accuracy:} Proportion of test samples for which the top predicted class matches the ground-truth label:
\[ \mathrm{Acc} = \frac{1}{N}\sum_{i=1}^{N}\mathbb{1}(\hat{y}_i = y_i)\]

\item \textbf{Macro F1-Score}: Per-class precision and recall are computed as:
    \[
    \text{P}_k = \frac{TP_k}{TP_k + FP_k}, \quad
    \text{R}_k = \frac{TP_k}{TP_k + FN_k}
    \]
    The macro F1 is the unweighted mean of per-class F1 scores:
    \[
    \text{Macro F1} = \frac{1}{K} \sum_{k=1}^{K}
    \frac{2 \cdot \text{P}_k \cdot \text{R}_k}{\text{P}_k + \text{R}_k}
    \]
    This metric treats all classes equally regardless of class size, making it robust to the moderate imbalance present in the dataset.
\end{enumerate}

\paragraph{Segmentation metrics}

SAM3 produces geometrically accurate contours when a detection occurs, so boundary-level metrics are not the primary focus. Instead, metrics target the two observed failure modes.

\begin{enumerate}
\item \textbf{Detection Rate}: fraction of images for which the decoder returns a non-empty mask:
\[  R_\mathrm{det} = \frac{1}{N}\sum_{i=1}^{N}\mathbb{1}\!\left(\textstyle\sum M_i > 0\right)\]

\item \textbf{Missing Interior Ratio} : fraction of the filled object area that is absent from the raw mask: 
\[ \rho_\mathrm{hole}(M) = \frac{\mathrm{Area}(M_\mathrm{filled})-\mathrm{Area}(M)}{\mathrm{Area}(M_\mathrm{filled})}\]
( where $M_\mathrm{filled} = \mathrm{binary\_fill\_holes}(M)$)

\item \textbf{Valid Rate}: fraction of images yielding a non-empty, internally coherent ($\rho_\mathrm{hole} < 0.1$), single-component mask:
\[  R_\mathrm{valid} = \frac{1}{N}\sum_{i=1}^{N}\mathbb{1}\!\left(M_i\!\neq\!\emptyset \;\land\; \rho_\mathrm{hole}\!<\!0.1 \;\land\; C(M_i)\!=\!1\right)\]


\item \textbf{Average Quality Score}: a continuous coherence score penalizing both holes and fragmentation:
\[  S_\mathrm{qual} = (1-\rho_\mathrm{hole})\times\frac{1}{C}\]
\end{enumerate}


==> sections_sam3/results.tex <==
\section{Results}

\subsection{Classification Results}

All experiments were evaluated on the stratified test set of 1,602 images. Table~\ref{tab:classification_results} compares frozen SAM2 and SAM3 encoders paired with different classification heads against an end-to-end ResNet-18 baseline.

\begin{table}[htbp]
\centering
\caption{Classification performance comparison across model configurations (All SAM-based encoders remain frozen)}
\label{tab:classification_results}
\begin{tabular}{llcc}
\hline
\textbf{Encoder (frozen)} & \textbf{Head} & \textbf{Top-1 Acc. (\%)} & \textbf{Macro F1} \\ 
\hline
SAM2 & MLP & 58.49 & 0.5448 \\
SAM2 & SLCA+MLP & 60.80 & 0.5729 \\ 
\hline
SAM2 & ResNet & 86.58 & 0.8545 \\
SAM2 & SLCA+ResNet & 86.58 & 0.8593 \\ 
\hline
SAM3 & ResNet & 94.51 & 0.9416 \\
SAM3 & SLCA+ResNet & \textbf{95.57} & \textbf{0.9523} \\
\hline
\multicolumn{2}{c}{ResNet-18 {\scriptsize (End-to-End)}} & \textbf{97.19} & \textbf{0.970} \\
\hline
\end{tabular}
\end{table}

\subsubsection{Foundation Model Feature Transfer}

A substantial performance gap is observed between SAM2 and SAM3 representations. While SAM2 enables significantly faster feature extraction ($9.7$ img/s), its downstream classification performance remains limited compared to SAM3. In contrast, SAM3, despite being approximately five times slower ($2.0$ img/s), consistently produces more discriminative features.

This difference can be attributed to the nature of the learned representations. SAM2 feature maps emphasize fine-grained local structures, preserving details such as striae-like textures and sharp contours. However, these features appear insufficient for robust class discrimination when used in isolation. Conversely, SAM3 produces more abstract and spatially diffuse representations, which better capture global semantic patterns relevant to taxonomic identity.

These results suggest that semantic richness outweighs local detail in this classification setting, particularly for visually similar classes where global morphology is more informative than texture alone.

\begin{figure}[htbp]
    \centering
    % --- Left Column (Original only) ---
    \begin{minipage}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/diatom.jpg}\\
        \vspace{2pt}
        {\scriptsize (a) Original}
    \end{minipage}
    \hfill
    % --- Center Column (SAM2) ---
    \begin{minipage}[b]{0.36\linewidth}
        \centering
        \includegraphics[width=0.46\linewidth]{images/sam2_1.png}\hspace{1pt}%
        \includegraphics[width=0.46\linewidth]{images/sam2_2.png}\\[1pt]
        \includegraphics[width=0.46\linewidth]{images/sam2_3.png}\hspace{1pt}%
        \includegraphics[width=0.46\linewidth]{images/sam2_4.png}\\
        \vspace{2pt}
        {\scriptsize (b) SAM2 features}
    \end{minipage}
    \hfill
    % --- Right Column (SAM3) ---
    \begin{minipage}[b]{0.36\linewidth}
        \centering
        \includegraphics[width=0.46\linewidth]{images/sam3_1.png}\hspace{1pt}%
        \includegraphics[width=0.46\linewidth]{images/sam3_2.png}\\[1pt]
        \includegraphics[width=0.46\linewidth]{images/sam3_3.png}\hspace{1pt}%
        \includegraphics[width=0.46\linewidth]{images/sam3_4.png}\\
        \vspace{2pt}
        {\scriptsize (c) SAM3 features}
    \end{minipage}
    
    \caption{Compact visual comparison: original input (left), and grayscale visualizations of some of the 256 extracted feature channels for SAM2 (center) and SAM3 (right)}
    \label{fig:feature_comparison_no_pre}
\end{figure}



\subsubsection{Impact of Classifier Head Design}

The architecture of the classification head plays a critical role in determining how effectively frozen features can be exploited.

\paragraph{Spatial Information Preservation.}
Standard MLP heads perform poorly, particularly with SAM2 features (58.49\% accuracy). This can be explained by the loss of spatial structure induced by flattening operations, which discard positional relationships between features. As a result, the classifier is unable to leverage the spatial organization inherent in the encoder outputs.

Replacing the MLP with a ResNet-style head leads to a dramatic improvement, increasing performance to over 86\% for SAM2 and above 94\% for SAM3. This highlights the importance of preserving spatial inductive biases when working with dense feature maps.

\paragraph{Effect of SLCA}

The introduction of the Spatially Localized Channel Attention (SLCA) mechanism provides a consistent and moderate performance gain across configurations. For SAM3, the SLCA+ResNet model achieves 95.57\% accuracy and a macro F1 score of 0.9523, narrowing the gap with the baseline.

This improvement suggests that SLCA enhances feature utilization by reweighting informative channels while maintaining spatial locality, leading to better class separation.

\subsubsection{Comparison with End-to-End Learning}

The fully supervised ResNet-18 baseline achieves the highest overall performance (97.19\% accuracy), confirming the advantage of end-to-end optimization when sufficient labeled data is available.

However, the SAM3-based models, particularly SAM3 + SLCA + ResNet, achieve competitive results while keeping the encoder frozen. The performance gap of less than 2\% demonstrates that foundation model features can serve as strong general-purpose representations, even without task-specific fine-tuning.

This highlights a favorable trade-off between performance and flexibility, as frozen encoders can be reused across tasks with minimal adaptation.

\subsubsection{Training Efficiency and Convergence}

Training efficiency varies significantly depending on the chosen architecture, as summarized in Table~\ref{tab:training_time_results}.

\begin{table}[htbp]
\centering
\caption{Training-time comparison across model configurations.}
\label{tab:training_time_results}
\begin{tabular}{lc}
\hline
\textbf{Model Configuration} & \textbf{Total Time (s)} \\
\hline
SAM2 + MLP & 3207.79 \\
SAM2 + SLCA + MLP & 3222.08 \\
\hline
SAM2 + ResNet & 825.93 \\
SAM2 + SLCA + ResNet & 825.49 \\
\hline
SAM3 + ResNet & 1646.07 \\
SAM3 + SLCA + ResNet & 1188.70 \\
\hline
ResNet-18 & 241.37 \\
\hline
\end{tabular}
\end{table}

Models based on MLP heads exhibit significantly slower convergence, requiring over 100 epochs to stabilize. This inefficiency further underscores their inability to effectively leverage spatial features.

In contrast, ResNet-based heads converge much faster and achieve higher performance, indicating a more efficient use of the extracted representations. Interestingly, the addition of SLCA slightly reduces training time in the SAM3 configuration, suggesting improved optimization dynamics.

Despite its superior accuracy, the end-to-end ResNet-18 model remains the most computationally efficient, achieving both the fastest training time and best performance. However, SAM3-based approaches provide a strong alternative when leveraging pretrained foundation models is desirable.


\subsection{Segmentation Results}


\subsubsection{Prompt Examples for \textit{Cyclostephanos dubius}}

To illustrate how the five prompt types differ in practice, Table~\ref{tab:prompt_example} shows all five variants for \textit{Cyclostephanos dubius}.

\begin{table}[htbp]
\centering
\caption{Prompt instantiations for \textit{Cyclostephanos dubius}}
\label{tab:prompt_example}
\begin{tabular}{p{2.5cm} p{5.0cm}}
\toprule
\textbf{Type} & \textbf{Prompt text} \\
\midrule
Minimal &
  \textit{``diatom''} \\[4pt]
Species Name &
  \textit{``Cyclostephanos dubius''} \\[4pt]
Simple Morphology &
  \textit{``a round centric diatom''} \\[4pt]
Detailed Morphology &
  \textit{``a circular centric diatom with a patterned valve face, featuring radial striae and a structured central area''} \\[4pt]
Noisy &
  \textit{``an elongated centric diatom with a patterned valve face, featuring radial striae and a structured central area''} \\
\bottomrule
\end{tabular}
\end{table}

This example illustrates the core design question studied here. The Simple Morphology prompts describes visually observable features (shape and symmetry) that SAM3 can ground in its learned representations. The Detailed Morphology prompt introduces precise but niche biological terminology. The Species Name prompt relies entirely on a taxonomic label absent from SAM3's pretraining data. The Noisy prompt introduces deliberate ambiguity to test robustness.

\subsubsection{Effect of Prompt Type on Segmentation Quality}

Table~\ref{tab:segmentation_results} reports structural segmentation metrics across all five prompt types. A clear trend emerges: shorter, visually grounded prompts yield better detection and structural quality, while greater specificity tends to hurt performance.

\begin{table}[htbp]
\centering
\caption{Structural segmentation metrics across prompt types.}
\label{tab:segmentation_results}
\begin{tabular}{lccc}
\toprule
\textbf{Prompt Type} & \textbf{Det.\ Rate} & \textbf{Valid Rate} & \textbf{Avg.\ Quality} \\
\midrule
Minimal              & 0.8464 & 0.8140 & 0.9863 \\
Simple Morphology    & \textbf{0.8664} & \textbf{0.8358} & 0.9853 \\
Detailed Morphology  & 0.6473 & 0.6292 & 0.9887 \\
Species Name         & 0.0050 & 0.0050 & 1.0000 \\
Noisy                & 0.6205 & 0.5999 & 0.9881 \\
\bottomrule
\end{tabular}
\end{table}

Simple Morphology prompts achieve the best results: detection rate of 0.8664 and valid rate of 0.8358. These prompts provide enough visual grounding to localize the diatom without over-constraining the decoder. Minimal prompts perform only slightly below, confirming that concise descriptions are preferable to elaborate ones.

Performance drops sharply as prompts grow more specific. Detailed Morphology prompts lower the detection rate to 0.6473, suggesting that dense biological vocabulary creates a mismatch with SAM3's internal representations and prevents reliable localization. Species Name prompts cause near-total failure: detection and valid rates both fall to 0.005. This confirms that SAM3 has no meaningful representation of diatom taxonomic names, since they were absent from its pretraining data. The few successful detections with species-name prompts achieve a perfect quality score of 1.0, but this is statistically irrelevant given the near-zero detection rate. Noisy prompts produce intermediate results, with degraded detection and validity relative to simple prompts.

\subsubsection{The Interior Hollowing Artifact}

A second systematic failure mode appears across all prompt types: some masks correctly trace the diatom boundary but leave the interior unsegmented, producing hollow or ring-like shapes. This occurs because diatom interiors have low contrast with the background in grayscale images. When the intensity difference between interior and background is small, the decoder focuses on high-gradient boundary regions and fails to assign interior pixels to the foreground.

The consistent gap between detection rate and valid rate in Table~\ref{tab:segmentation_results} reflects this effect. Hollow masks are counted as detected but fail the validity criterion . The gap quantifies the proportion of detections that are structurally incomplete.

Qualitative examples of both failure modes are shown in Figure~\ref{fig:prompt_masks}.

\begin{figure}[htbp]
\centering
\begin{tabular}{cccccc}
(a) & (b) & (c) & (d) & (e) & (f) \\[4pt]
\includegraphics[width=0.12\linewidth]{images/24_roi_1.jpg} &
\includegraphics[width=0.12\linewidth]{images/24_roi_1_minimal.png} &
\includegraphics[width=0.12\linewidth]{images/24_roi_1_simple.png} &
\includegraphics[width=0.12\linewidth]{images/24_roi_1_detailed.png} &
\includegraphics[width=0.12\linewidth]{images/24_roi_1_species_name.png} &
\includegraphics[width=0.12\linewidth]{images/24_roi_1_noisy.png} \\[2pt]
\includegraphics[width=0.12\linewidth]{images/38_roi_4.jpg} &
\includegraphics[width=0.12\linewidth]{images/38_roi_4_minimal.png} &
\includegraphics[width=0.12\linewidth]{images/38_roi_4_simple.png} &
\includegraphics[width=0.12\linewidth]{images/38_roi_4_detailed.png} &
\includegraphics[width=0.12\linewidth]{images/38_roi_4_species_name.png} &
\includegraphics[width=0.12\linewidth]{images/38_roi_4_noisy.png} \\[2pt]
\includegraphics[width=0.12\linewidth]{images/37_roi_7.jpg} &
\includegraphics[width=0.12\linewidth]{images/37_roi_7_minimal.png} &
\includegraphics[width=0.12\linewidth]{images/37_roi_7_simple.png} &
\includegraphics[width=0.12\linewidth]{images/37_roi_7_detailed.png} &
\includegraphics[width=0.12\linewidth]{images/37_roi_7_species_name.png} &
\includegraphics[width=0.12\linewidth]{37_roi_7_noisy.png} \\
\end{tabular}
\caption{Segmentation results across five prompt types for three representative specimens. (a)~Original; (b)~Minimal; (c)~Simple Morphology; (d)~Detailed Morphology; (e)~Species Name; (f)~Noisy. Empty panels in column~(e) illustrate the near-total detection failure of species-name prompts.}
\label{fig:prompt_masks}
\end{figure}

\subsubsection{Generalization to Multi-Diatom Slides}

To evaluate robustness beyond the single-diatom controlled setting, Simple Morphology prompts were applied to slides containing multiple diatom individuals of different species. The model successfully detected and segmented all diatoms present in the slide.

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/1.jpg}
        \centerline{(a)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/3 (1).jpg}
        \centerline{(b)}
    \end{minipage}
    \caption{Zero-shot segmentation on multi-diatom slides}
    \label{fig:multi_diatom_results}
\end{figure}
